Is Data Valuation Learnable and Interpretable?

Measuring the value of individual samples is critical for many data-driven tasks, e.g., the training of a deep learning model. Recent literature witnesses the substantial efforts in developing data valuation methods. The primary data valuation methodology is based on the Shapley value from game theory, and various methods are proposed along this path. {Even though Shapley value-based valuation has solid theoretical basis, it is entirely an experiment-based approach and no valuation model has been constructed so far.} In addition, current data valuation methods ignore the interpretability of the output values, despite an interptable data valuation method is of great helpful for applications such as data pricing. This study aims to answer an important question: is data valuation learnable and interpretable? A learned valuation model have several desirable merits such as fixed number of parameters and knowledge reusability. An intrepretable data valuation model can explain why a sample is valuable or invaluable. To this end, two new data value modeling frameworks are proposed, in which a multi-layer perception~(MLP) and a new regression tree are utilized as specific base models for model training and interpretability, respectively. Extensive experiments are conducted on benchmark datasets. {The experimental results provide a positive answer for the question.} Our study opens up a new technical path for the assessing of data values. Large data valuation models can be built across many different data-driven tasks, which can promote the widespread application of data valuation.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Computer Society subset of the full IEEEtran
package and is intended for use with IEEE Computer Society publications.
The included version of the IEEEtran_HOWTO.pdf has been specially formatted
in IEEE Computer Society (compsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf_compsoc.tex, bare_jrnl_compsoc.tex.
***************************************************************************


==> ref.tex <==
% Generated by IEEEtran.bst, version: 1.14 (2015/08/26)
\begin{thebibliography}{10}

\bibitem{OAU2023}
K.~F. Jiang, W.~Liang, J.~Zou, and Y.~Kwon, ``Opendataval: a unified benchmark for data valuation,'' in \emph{NeurIPS}, 2023.

\bibitem{ASODP2022}
J.~Pei, ``A survey on data pricing: From economics to data science,'' \emph{IEEE Transactions on Knowledge and Data Engineering}, vol.~34, no.~10, pp. 4586--4608, 2022.

\bibitem{DSE2019}
A.~Ghorbani and J.~Zou, ``Data shapley: Equitable valuation of data for machine learning,'' in \emph{arXiv:1904.02868}, 2019.

\bibitem{AVF1953}
L.~S. Shapley, ``A value for n-person games,'' in \emph{In Contributions to the Theory of Games}, 1953, pp. 307--317.

\bibitem{DVUR2020}
J.~Yoon, S.~Arik, and T.~Pfister, ``Data valuation using reinforcement learning,'' in \emph{ICML}, 2020, pp. 10\,842--10\,851.

\bibitem{MIE2022}
J.~Lin, A.~Zhang, M.~L{\'e}cuyer, J.~Li, A.~Panda, and S.~Sen, ``Measuring the effect of training data on deep learning predictions via randomized experiments,'' in \emph{ICML}, 2022, pp. 13\,468--13\,504.

\bibitem{TED2019}
R.~Jia, D.~Dao, B.~Wang, F.~A. Hubis, N.~Hynes, N.~M. G\"{u}rel, B.~Li, C.~Zhang, D.~Song, and C.~J. Spanos, ``Towards efficient data valuation based on the shapley value,'' in \emph{AISTAS}, 2019, pp. 1167--1176.

\bibitem{UBP2017}
P.~W. Koh and P.~Liang, ``Understanding blackbox predictions via influence functions,'' in \emph{ICML}, 2017, p. 1885–1894.

\bibitem{BSA2022}
Y.~Kwon and J.~Zou, ``Beta shapley: a unified and noise-reduced data valuation framework for machine learning,'' in \emph{AISTATS}, 2022.

\bibitem{ATE2023}
H.~Chen, I.~C. Covert, S.~M. Lundberg, and S.-I. Lee, ``Algorithms to estimate shapley value feature attributions,'' \emph{Nature Machine Intelligence}, vol.~5, pp. 590--601, 2023.

\bibitem{TMS2020}
M.~Sundararajan and A.~Najmi, ``The many shapley values for model explanation,'' in \emph{ICML}, 2020, pp. 9269--9278.

\bibitem{AFAE2023}
Y.~Chai, R.~Liang, S.~Samtani, H.~Zhu, M.~Wang, Y.~Liu, and Y.~Jiang, ``Additive feature attribution explainable methods to craft adversarial attacks for text classification and text regression,'' \emph{IEEE Transactions on Knowledge and Data Engineering}, vol.~35, no.~12, pp. 12\,400--12\,414, 2023.

\bibitem{IMS2021}
H.~Zhang, Y.~Xie, L.~Zheng, D.~Zhang, and Q.~Zhang, ``Interpreting multivariate shapley interactions in dnns,'' in \emph{AAAI}, 2021, pp. 10\,877--10\,886.

\bibitem{HCA2023}
L.~Chen, S.~Lou, K.~Zhang, J.~Huang, and Q.~Zhang, ``Harsanyinet: Computing accurate shapley values in a single forward propagation,'' in \emph{arXiv:2304.01811}, 2023.

\bibitem{wu2023data}
O.~Wu and R.~Yao, ``Data optimization in deep learning: A survey,'' \emph{arXiv preprint arXiv:2310.16499}, 2023.

\bibitem{SAG2020}
T.~Castells, P.~Weinzaepfel, and J.~Revaud, ``Superloss: A generic loss for robust curriculum learning,'' in \emph{NeurIPS}, 2020, pp. 4308--4319.

\bibitem{SPLA2017}
Y.~Fan, R.~He, J.~Liang, and B.~Hu, ``Self-paced learning: an implicit regularization perspective,'' in \emph{AAAI}, 2017, pp. 1877--1883.

\bibitem{PDA2008}
Q.~A. Wang, ``Probability distribution and entropy as a measure of uncertainty,'' \emph{Journal of Physics A: Mathematical and Theoretical}, vol.~41, no.~6, p. 065004, 2008.

\bibitem{ACSOF2023}
Z.~Wang, E.~Yang, L.~Shen, and H.~Huang, ``A comprehensive survey of forgetting in deep learning beyond continual learning,'' in \emph{arXiv2307.09218}, 2023.

\bibitem{DAN2017}
N.~Frosst and G.~Hinton, ``Distilling a neural network into a soft decision tree,'' in \emph{arXiv:1711.09784}, 2017.

\bibitem{NBDT}
A.~Wan, L.~Dunlap, D.~Ho, J.~Yin, S.~Lee, H.~Jin, S.~Petryk, S.~Bargal, and J.~Gonzalez, ``Nbdt: neural-backed decision trees,'' in \emph{ICLR}, 2021, pp. 1--12.

\bibitem{ITS2023}
X.~Zhou, O.~Wu, and M.~Li, ``Investigating the sample weighting mechanism using an interpretable weighting framework,'' \emph{IEEE Transactions on Knowledge and Data Engineering}, pp. 1--14, 2023.

\bibitem{DNDT}
Y.~Yang, I.~G. Morillo, and T.~M. Hospedales, ``Deep neural decision trees,'' in \emph{arXiv:1806.06988}, 2018.

\bibitem{SKC2021}
Z.~Han, X.~Yuan, C.~Xu, S.~Jiang, and X.~Wang, ``Sparse kronecker-product coding for unsourced multiple access,'' \emph{IEEE Wireless Communications Letters}, vol.~10, no.~10, pp. 2274--2278, 2021.

\bibitem{ETD2019}
R.~Jia, D.~Dao, B.~Wang, F.~A. Hubis, N.~M. Gurel, B.~Li, C.~Zhang, C.~Spanos, and D.~Song, ``Efficient task-specific data valuation for nearest neighbor algorithms,'' in \emph{Proceedings of the VLDB Endowment}, 2019, pp. 1610--1623.

\bibitem{VFA2021}
X.~Xu, Z.~Wu, C.~S. Foo, and B.~K.~H. Low, ``Validation free and replication robust volume-based data valuation,'' in \emph{NerIPS}, 2021, pp. 10\,837--10\,848.

\bibitem{DBA2023}
J.~T. Wang and R.~Jia, ``Data banzhaf: A robust data valuation framework for machine learning,'' in \emph{AISTATS}, 2023, pp. 6388--6421.

\bibitem{LDV2023}
H.~A. Just, F.~Kang, T.~Wang, Y.~Zeng, M.~Ko, M.~Jin, and R.~Jia, ``Lava: Data valuation without pre-specified learning algorithms,'' in \emph{ICLR}, 2023.

\bibitem{DOE2023}
Y.~Kwon and J.~Zou, ``Data-oob: Out-of-bag estimate as a simple and efficient data value,'' in \emph{ICML}, 2023, pp. 18\,135--18\,152.

\bibitem{Krizhevsky32}
A.~Krizhevsky and G.~Hinton, ``Learning multiple layers of features from tiny images,'' 2009.

\bibitem{LWC2011}
A.~Maas, R.~E. Daly, P.~T. Pham, D.~Huang, A.~Y. Ng, and C.~Potts, ``Learning word vectors for sentiment analysis,'' in \emph{ACL}, 2011, pp. 142--150.

\bibitem{PST2006}
D.~Greene and P.~Cunningham, ``Practical solutions to the problem of diagonal dominance in kernel document clustering,'' in \emph{ICML}, 2006, pp. 377--384.

\bibitem{ImageNet0FeifeiLi}
O.~Russakovsky, J.~Deng, H.~Su, J.~Krause, S.~Satheesh, S.~Ma, Z.~Huang, A.~Karpathy, A.~Khosla, M.~Bernstein, A.~C. Berg, and L.~Fei-Fei, ``Imagenet large scale visual recognition challenge,'' \emph{Int. J. Comput. Vision}, vol. 115, no.~3, p. 211–252, 2015.

\end{thebibliography}


